PayPlace: Secure and Flexible Operator-Mediated Payments in Blockchain Marketplaces at Scale

Decentralized marketplace applications demand fast, cheap and easy-to-use cryptocurrency payment mechanisms to facilitate high transaction volumes. The standard solution for off-chain payments, state channels, are optimized for frequent transactions between two entities and impose prohibitive liquidity and capital requirements on payment senders for marketplace transactions. We propose PayPlace, a scalable off-chain protocol for payments between consumers and sellers. Using PayPlace, consumers establish a virtual unidirectional payment channel with an intermediary operator to pay for their transactions. Unlike state channels, however, the PayPlace operator can reference the custodial funds accrued off-chain in these channels to in-turn make tamper-proof off-chain payments to merchants, without locking up corresponding capital in channels with merchants. Our design ensures that new payments made to merchants are guaranteed to be safe once notarized and provably mitigates well-known drawbacks in previous constructions like the data availability attack and ensures that neither consumers nor merchants need to be online to ensure continued safety of their notarized funds. We show that the on-chain monetary and computational costs for PayPlace is O(1) in the number of payment transactions processed, and is near-constant in other parameters in most scenarios. PayPlace can hence scale the payment throughput for large-scale marketplaces at no marginal cost and is orders of magnitude cheaper than the state-of-art solution for non-pairwise off-chain payments, Zero Knowledge Rollups.

==> Background.tex <==
\section{Marketplace Payments with Existing Designs}
\label{sec:existing}
\label{sec:background}

We first construct a simple model for operator-mediated marketplace payments using pairwise channels between the operator and consumers/service providers. Next, we demonstrate a Plasma-style sidechain solution (based on MoreVP~\cite{morevp}) that involves periodic transaction notarizations on the root chain. %
In Section~\ref{sec:model}, we show that \name{} utilizes a modified construction of the first model for facilitating a part of the sidechain, and improves on Plasma-style constructions by addressing their security challenges. %
For the rest of this article, we use \currency{} to denote the cryptocurrency denomination in use, e.g. ETH. Appendix~\ref{sec:systemNotation} summarizes our notation.


\subsection{Using Pairwise Payment Channels}
\label{sec:pairwisePayment}
A consumer $c$ with public key $pk_{c}$ %
deposits \currency{} in the smart-contract, to be spent incrementally in payments to the operator $\omega$ for orders \change{they place}{that she places} in the marketplace. \change{Their}{The} deposit establishes a pairwise payment channel %
with $\omega$. In our case, it suffices if the channel is unidirectional since payments flow from the consumer to the operator; hence the consumer need not be \textit{always online} to guard against operator malfeasance since she is not owed any funds in this channel (with refunds and returns as external to the protocol).%


An off-chain payment from $c$ for an order consists of a transaction $T = (\mu, pk_\omega, pk_{c})$, where $\mu$ is the payment amount denominated in \currency{} and the recipient is the operator with public key $pk_\omega$, and the digital signature of the transaction $\sigma = \mathcal{S}(T, sk_c)$, which the consumer generates using their private key $sk_{c}$. 
Since the consumer-operator payment channel is unidirectional, the amount $\mu$ specified in $T$ indicates the \emph{total} amount promised by the consumer to the operator as of when %
$T$ is generated, incorporating the incremental amount the consumer intends to pay for their latest order in the marketplace. Hence, $\mu$ is the total amount of the consumer's funds in the channel that is owned by the operator as of this transaction. 
We let $s(T)$ and $\mu(T)$ denote the sending consumer's public key $pk_c$ and amount $\mu$ specified in transaction $T$ respectively.
The consumer may deposit more \currency{} at any time for use in the marketplace. We therefore use $D_{c, t}$ and $\mu_{c,t}^\ast$ to denote the total funds deposited and spent (in off-chain payments with the operator), respectively, by consumer $c$ as of \change{}{time} $t$.
Note that the operator knows the deposited funds $D_{c,t}$ since deposits and top-ups (as well as withdrawals) happen through the contract on the root chain, which stores and updates $D_{c,t}$ for each consumer. %
The operator verifies \change{such}{}an off-chain payment transaction $T$ sent by consumer~$c$ at time $t$ by evaluating if the sender has sufficient balance to make this transaction (i.e. $\mu(T) \leq D_{c,t}$) and ensuring that the operator balance in $c$'s payment channel only increases as a result of $T$ (i.e. $\mu_{c,t}^\ast \leq \mu(T)$) thereby ensuring payment unidirectionality. The operator also verifies the digital signature $\sigma$ with verification function $\mathcal{V}$; $\mathcal{V}(pk_c, T, \sigma)=1$ if $sk_c$ was used to sign $T$ to yield $\sigma$.%

To forward these consumer payments to providers (who may be assigned at the time of order placement \change{itself}{} or later on), the operator generates new transactions that make payment promises to to each appropriate provider $p$. %
To do so, the operator establishes a unidirectional payment channel with each provider and deposits sufficient funds in each for relaying later payments. An off-chain payment transaction from the operator to a provider $p$ is then defined as $T'=(\mu', pk_p, pk_\omega)$, sourced from the funds deposited by the operator $\omega$ in his channel with $p$, along with the associated signature. Similar to $T$, the specified $\mu'$ in $T'$ represents the total amount of the operator's funds in this channel that is owned by the provider as of this transaction. %
To withdraw these funds, the recipient (operator or provider) simply provides the last signed off-chain transaction received from the sender to the contract.

A significant drawback of this model is the high liquidity requirements it imposes on the operator, 
who must forecast the estimated payouts to each provider and deposit sufficient \currency{} in each channel so as to minimize the root chain transactions (which incur fees and time) involved in adding more funds to the channel. This requirement arises because funds from consumers' payments in the pairwise channels are not accessible for use with others until the operator initiates a root chain transaction to transfer the funds to their address. Hence, we now provide a formalization of Plasma-style sidechains for operator-mediated marketplace payments, where operators can directly forward payments they receive from consumers to providers. The \name{} protocol utilizes aspects of pairwise payment channels and Plasma-style sidechains (discussed below) to enable secure marketplace transactions at scale.

\vspace{-1em}
\subsection{Using Plasma-style Sidechains}
\label{sec:plasmaStyle}
In the more general sidechain model, deposits in the smart-contract %
can be used to pay any participant of the sidechain (i.e., consumers /providers/the operator). Since we \change{continue to be}{are} interested in operator-mediated marketplace transactions, we characterize a model where consumers use their deposits to make payments using the sidechain to the operator (e.g., at the time of order placement) and the operator in turn makes payments to providers using the sidechain as well (note that the marketplace operator is also the sidechain operator). %

Let time be discretized and the resulting points in time be indexed by $t = 1,2,\ldots$. %
Consumers' deposits of \currency{} in the contract %
are realized as Unspent Transaction Outputs (UTXOs)~\cite{delgado2018analysis} in the sidechain. An off-chain payment transaction from a consumer to the operator then specifies the payment amount (i.e. the incremental amount corresponding to the order placed by the consumer), the recipient $pk_\omega$, and a reference to UTXO that the consumer owns and wishes to use for this off-chain transaction. %
Unlike the simpler payment channels, an off-chain transaction received in the sidechain is not immediately guaranteed to be available for use by the recipient until the transaction is \textit{notarized in a Plasma block}.%

We now describe the generation and notarization process of a Plasma block. The operator periodically generates a \textit{Plasma block} \change{$\kappa$}{} every $t_a$ time slots, containing all the signed payment transactions that have transpired off-chain since the last notarized \change{one}{block} was generated. A Plasma block is defined by $\kappa = (\mathbb{T}, \mathcal{M})$ where $\mathbb{T}$ contains the off-chain payment transactions arranged by some ordering and $\mathcal{M}$ is the Merkle tree with leaves corresponding to hashes of the transactions in $\mathbb{T}$. The operator then generates a \textit{short commitment to the Plasma block $\kappa$}, which contains information that the Plasma contract on the root chain uses to notarize the sidechain transaction activity corresponding to $\kappa$. For the main Plasma constructions~\cite{mvp, morevp}, this commitment is simply the root of the Merkle tree $\mathcal{M}$, which is short and avoid the excess storage costs that would be incurred if the entire transaction activity were to be individually verified on-chain. The operator submits this commitment to the smart-contract which simply stores it. %
We denote by $\mathbb{K}_{t}$ %
the set of Plasma blocks corresponding to accepted commitments as of time $t$, \textit{ordered by the times they were accepted}, with $\mathbb{K}_{t}(-1)$, $\mathbb{K}_{t}(-2)$, $\dots$ denoting the latest accepted block, the previous accepted block, and so on. Once a consumer's off-chain payment is included in a notarized Plasma block, the operator may similarly generate an off-chain payment to providers that references UTXOs that the operator now owns as a result of the consumers' notarized payment.

To withdraw funds from the sidechain, a user must provide a Merkle proof showing that a valid transaction (signed by the previous owner of the funds) assigning them their UTXO has been included in one of the committed Plasma blocks. We use $\mathbb{T}_p(\kappa)$ (and by extension, $\mathbb{T}_\omega(\kappa)$) to denote the set of off-chain payment transactions included in Plasma block $\kappa$ that assigned funds to provider $p$ (or the operator $\omega$).
Hence, a valid off-chain payment transaction received on the sidechain \change{are}{constitutes} funds available for subsequent use by the recipient only when it is included in $\mathbb{T}_p(\kappa)$ where $\kappa$ is a block whose commitment (i.e., Merkle root) has been notarized on the root chain.
However, \change{such a withdrawal}{this} process allows a participant (e.g., the operator) to maliciously withdraw UTXOs assigned to them in a notarized Plasma block that are spent in subsequent Plasma blocks (e.g., to pay providers). Hence, the contract imposes a \textit{challenge period} on withdrawals, during which anyone may contest the withdrawal by showing a Merkle proof that the UTXO in question has been spent in a subsequently notarized block. 

This model exposes consumers as well as providers %
to malicious attacks from the operator. 
Both consumers (whose deposited funds are now UTXOs in the sidechain) and providers (who are assigned UTXOs in the sidechain as payments by the operator) risk losing their funds %
if the operator inserts \textit{invalid out-of-nowhere} transactions in a block~\cite{mvp}. %
These withdrawals may be detected as valid, and the operator can drain the contract of funds. This generic sidechain design, when applied to marketplaces, also \change{results in provider exposure}{exposes providers} to counter-consumer risk. Consumers, like operators, may attempt to withdraw spent UTXOs. Existing protocols prevent this by allowing older UTXOs to be exited first when a withdrawal is initiated~\cite{morevp}, but such a solution results \textit{mass exits} that flood the root chain with a high volume of exit transactions, leading also to high transaction fees. Even so, to contest the withdrawal of a spent UTXO or to proactively exit when the operator includes an out-of-nowhere transaction, consumers and providers must be \textit{online} to monitor side-chain activity and submitted exits. Finally, the operator may well commit a hash to the root chain, \textit{without revealing the corresponding Plasma block to the sidechain participants}. This \textit{data availability attack} leaves consumers and providers unsure of what transactions were included in a committed Plasma block, forcing them to withdraw their funds (in case the operator had inserted malicious transactions) and resulting in mass exits.  %

Since there are no checks performed by the contract to verify that the transactions included in a commitment are valid and to protect against these attacks, this design poses risks to funds that providers and consumers have on the sidechain, unless they are always online to detect potential malicious activity and react proactively. %



==> PlasmaGoModel.tex <==
\section{\name{} Model}
\label{sec:plasmaGoModel}
We extend the generic framework for marketplace sidechains introduced previously with notations that capture \name{}-specific interactions, which allows us to explain the protocol subsequently in Section~\ref{sec:protocol}.

\subsection{Assumptions} We assume the root chain supports BLS signature~\cite{boneh2018compact} verification and other relevant operations like multiplication in group $\mathbb{G}_2$ where BLS public keys live. 
BLS is currently being standardized~\cite{blsDraft}. BLS curves are already in use~\cite{blsIssueZCash}, and Ethereum is expected to support BLS curves and avail BLS functionality such as key aggregation with its Casper release~\cite{blsPragmaticAggr}. 
We use the multiplicative notation for groups in this paper and references to signatures in \name{} implicitly mean BLS signatures.

==> RelatedWork.tex <==
\section{Related Work}
\label{sec:related}
State channels are a widely used mechanism in which repeated transactions %
between two users impose no marginal cost once some initial overhead is incurred in setting up and depositing funds %
into a pairwise channel between them. Such channels were first proposed for Bitcoin~\cite{decker2015fast} and are used, e.g., by %
Raiden Network~\cite{raiden}. Such pairwise channels are not sufficient for marketplaces where consumers may connect with unknown providers for only a few payments. %
Other designs~\cite{miller2017sprites, sivaraman2018routing} facilitate transactions between users without a direct payment channel by routing the payment through shared intermediary channels. However, in large decentralized marketplaces with sporadically online users, such routes may not exist for some consumer-provider pairs. Further, the intermediaries must commit funds to the route's outgoing channel, which then cannot be used to pay other users. Indeed, recent work has exposed incentive compatibility issues with such intermediaries ~\cite{beres2019cryptoeconomic}.%

Sidechains, on the other hand, enable uses well beyond pairwise payments. Sidechains broadly refer to off-chain payment protocols that involve periodic notarization of off-chain payment activity on a smart-contract on the root chain. Rules encoded in the contract would ideally validate or ``notarize" the transactions corresponding to the commitment, secure \vendors{}' resulting balances, and allow \vendors{} to withdraw \change{it}{them} by directly making calls to the contract. \iMadhu{Mention BFT vs centralized}Proposed designs~\cite{johnson2019sidechains, adler2019building} are in various stages of completeness and development, some similar to payment channels (e.g., Plasma Debit~\cite{debit} and Plasma Cash~\cite{cash}). Most sidechains are similar to the originally proposed Plasma-style sidechains~\cite{poon2017plasma}, with Minimum Viable Plasma~\cite{mvp} and its improved version More Viable Plasma ~\cite{morevp} as one of the earliest constructions to use periodic root chain notarization of off-chain payment transactions using \textit{short} commitments. 
The recently proposed Zero-Knowledge Rollup~\cite{zkrollup} significantly differs from these. With this, the sidechain operator computes a succinct non-interactive argument of knowledge (zkSNARK)~\cite{ben2014succinct, maller2019sonic} to prove to the smart-contract that each off-chain payment transaction included in the proof is legitimate (signed correctly with valid balances) \textit{without requiring validation of each transaction individually by smart-contract}. Certain zkSNARK techniques attractively enable %
proof verification in constant time, i.e., independent of the number of transactions in this case. ZK Rollups have garnered much recent interest; Ethereum's eighth major network update~\cite{istanbul} recently implemented changes that specifically optimize zkSNARK functionality. 
We show that \name{} can be several orders of magnitude cheaper than ZK Rollup.\iMadhu{cite Snappy here on in Intro}


==> SecurityAnalysis.tex <==
\section{Security Analysis}
\label{sec:analysis}
We now provide an overview \name{}'s security properties (proofs in Appendix~\ref{sec:proofs}).


\begin{lem}
\label{lem:useOwnKey}
In \name{}, a public key $pk_p$ can  be registered only by its owner $p$ (who knows $sk_p$). Further, unless $p$ colludes with the operator, she can  register $pk_p$ only once.
\end{lem}


